MonoSDF: Exploring Monocular Geometric Cues for Neural Implicit Surface Reconstruction

In recent years, neural implicit surface reconstruction methods have become popular for multi-view 3D reconstruction. In contrast to traditional multi-view stereo methods, these approaches tend to produce smoother and more complete reconstructions due to the inductive smoothness bias of neural networks. State-of-the-art neural implicit methods allow for high-quality reconstructions of simple scenes from many input views. Yet, their performance drops significantly for larger and more complex scenes and scenes captured from sparse viewpoints. This is caused primarily by the inherent ambiguity in the RGB reconstruction loss that does not provide enough constraints, in particular in less-observed and textureless areas. Motivated by recent advances in the area of monocular geometry prediction, we systematically explore the utility these cues provide for improving neural implicit surface reconstruction. We demonstrate that depth and normal cues, predicted by general-purpose monocular estimators, significantly improve reconstruction quality and optimization time. Further, we analyse and investigate multiple design choices for representing neural implicit surfaces, ranging from monolithic MLP models over single-grid to multi-resolution grid representations. We observe that geometric monocular priors improve performance both for small-scale single-object as well as large-scale multi-object scenes, independent of the choice of representation.

==> introduction_backup.tex <==
\section{Introduction}
3D reconstruction from multi-view images is a fundamental problem in computer vision with emerging applications such as graphics, animation, virtual reality, and more. \torsten{Why emerging? Aren't applications of 3D reconstruction, e.g., building 3D models for robotic navigation, for cultural heritage, as assets for games and movies, etc., well established?}
Recently, neural radiance fields (NeRFs)~\cite{Mildenhall2020ECCV} have shown impressive results on the task of novel view synthesis by using multi-layer perceptrons (MLPs) in combination with volume rendering techniques.
Building on NeRF, several works~\cite{Oechsle2021ICCV,Wang2021NEURIPS,Yariv2021NEURIPS} investigate how proposed techniques can be used for the task of 3D reconstruction and they introduce new ways \torsten{"new ways" sounds a bit handwavy, can we be more precise?} of modelling volume density as a function of the underlying 3D surface, which in turn improves optimized scene geometry. 
For example, in UNISURF~\cite{Oechsle2021ICCV} NeRF's density field is replaced by an occupancy field, while in NeuS~\cite{Wang2021ARXIVb} and VolSDF~\cite{Yariv2021NEURIPS} the density field is modeled with a signed distance field instead.
These methods show improved surface reconstruction quality compared to NeRF and the extracted meshes are smoother and more complete compared to traditional methods like COLMAP~\cite{Schoenberger2016CVPR} \torsten{maybe the latter is due to parameter settings? what about MVS methods that use learning only for components, e.g., depth map computation or predicting uncertainty for the depth, these are the current state of the art on tanks and temples and eth 3d.}.
However, all of these methods require a long optimization time and are limited to small scenes focusing on reconstructing single objects. %
\torsten{I think this paragraph jumps into details too quickly. I think it would be good to stay on a high level here and go into details in the next paragraph.}

Most recently, another line of research~\cite{Sun2021ARXIV,Yu2021cARXIV,Muller2022ARXIV} significantly reduces the training time of NeRF by replacing the large MLP  \torsten{the MLP was never mentioned before and might be confusing to readers not too familiar with NeRFs and neural scene representations.} with either dense voxel grids or a lightweight MLP conditioned on features distributed on a spatial 3D grid, which is cheap to query using trilinear interpolation. While these methods achieve comparable or even better novel view synthesis results compared to NeRF, and can represent sophisticated object shapes when dense 3D supervision are avaliable (\ie Instant-ngp~\cite{Muller2022ARXIV} and NGLOD~\cite{takikawa2021nglod}), it remains unclear how effective they can be as a general-purpose neural implicit surface representation trained only on multi-view RGB images as input. \TS{This seems a bit vague, can we at least explain why they are unlikely to handle more complex / larger scenes?}
\TS{I guess this paragraph will go in the new structure?}

In this work, we propose \textit{InstantSDF}, a neural implicit field conditioned on a multi-resolution feature grid \michael{change name? If so, not only inspired by Instant NGP}.
InstantSDF enables detailed large-scale 3D reconstruction from only multi-view posed images while also being more efficient to train compared to previous approaches. \torsten{I wouldn't call it large-scale since we are still looking at rather small scenes. Medium-scale might be more accurate. I would reserve large-scale for larger outdoor scenes. Also, wasn't there some work by NVidia on implicit neural representations for larger scenes? Also, BlockNerf handles larger scenes as well.} %
Our key observation is that a single, large MLP is insufficient to represent high-detail geometry while being computational expensive to evaluate and optimize.
In contrast, a high-resolution signed distance grid is cheap to evaluate with trilinear interpolation.
However, in contrast to an MLP-based representation, gradient updates only affect the local grid cell and have no influence on neighbouring areas. As a result, the optimization is more local leading to noisy geometry predictions in less-observed areas.
Using a small MLP together with a feature grid is a compromise between the two extremes.
While it is comparably efficient to optimize and evaluate due to the feature grid, it utilizes a shared MLP for all feature grid cells, thereby inheriting the favorable inductive biases of MLP-based representations.
However, this combination alone still leads to noisy geometry predictions with block-like artifacts as only a single, high-frequency grid is used.
Instead, we propose to combine grid features from multiple resolutions leading to an automatic balance of low and high frequencies and provide a detailed analysis of the unique properties of multi-resolution grids. \zehao{do we need to add details here and what is the experiments to show?} We use surface-based volume rendering to optimize our model~\cite{Yariv2021NEURIPS} where sampling points around the surface is essential for optimization. We propose a simple gradient-guided sampling method to improve the sampling efficiency. Our key idea is to use the gradient of SDF along the ray to interpolate SDF values between ray points. Our sampling method only needs to evaluate 10 percent of points compared to VolSDF's sampling method and is thus much faster.
\andreas{can we make this more clear?}

\zehao{huge progress in monocular depth normal prediction but is not exploited in the context of multi-view surface reconstruction; ambiguity is hard to solve with pure rgb loss, matching loss, textureless region and rarely observed region. hopefully speed up the training}
While our method achieves better results than competing methods, we find it struggle when scaling to large scale complex scenes (\ie the advanced scenes in Tanks and Temples dataset\cite{Knapitsch2017SIGGRAPH}). Therefore, we propose to incorporate monocular geometric cues~\cite{Eftekhar_2021_ICCV} to guide the optimization. Specifically, we extract monocular geometric prior (\ie depth and surface normal) for each image and used it as an additional supervision for our optimization.\zehao{need more motivation for the monocular prior} In summary, we make the following contributions:

\begin{itemize}
    \item We present Instant SDF, a neural implicit surface reconstruction method utilizing multi-resolution feature grids. Our method enables detailed 3D reconstruction of large-scale scenes and is more efficient to optimize compared to state-of-the art implicit surface reconstruction methods. We provide a detailed analysis and deepened understanding of the effect of the multi-resolution feature grids.
    \item We introduce a general monocular geometric prior to improve the reconstruction quality and efficiency and scale the large scale scenes. We further show our geometric prior can significant boost the performance of other methods (\ie VolSDF~\cite{Yariv2021NEURIPS}). 
    \item We propose a simple yet efficient sampling algorithm based on the local gradient of the signed distance field along the ray. Our sampling algorithm is X times faster than VolSDF's error-bounded sampling. Further, our sampling method is generic and can also be incorporated into error-bounded sampling algorithm in VolSDF.
    \item We validated the effectiveness, efficiency and scalability of our Instant-SDF on the multiple challenging datasets, ranging from laboratory captured dataset(\ie the DTU dataset\cite{Aanes2016IJCV}) to large scale scenes (\ie the Tanks and Temples dataset\cite{Knapitsch2017SIGGRAPH}). \ We observe that our method yields higher geometric quality while converging faster than competing methods.
\end{itemize}

\section{Introduction1 - multi-res grid}
3D reconstruction from multi-view images is a fundamental problem in computer vision with well-established applications such as graphics, animation, virtual reality, and more. Recently, neural radiance fields (NeRFs)~\cite{Mildenhall2020ECCV} have shown impressive results on the task of novel view synthesis by using multi-layer perceptrons (MLPs) in combination with volume rendering techniques.
Building on NeRF, several works~\cite{Oechsle2021ICCV,Wang2021NEURIPS,Yariv2021NEURIPS} investigate how proposed techniques can be used for the task of 3D reconstruction and they introduce new ways \torsten{"new ways" sounds a bit handwavy, can we be more precise?} of modelling volume density as a function of the underlying 3D surface, which in turn improves optimized scene geometry. 
For example, in UNISURF~\cite{Oechsle2021ICCV} NeRF's density field is replaced by an occupancy field, while in NeuS~\cite{Wang2021ARXIVb} and VolSDF~\cite{Yariv2021NEURIPS} the density field is modeled with a signed distance field instead.
These methods show improved surface reconstruction quality compared to NeRF and the extracted meshes are smoother and more complete compared to traditional methods like COLMAP~\cite{Schoenberger2016CVPR} \torsten{maybe the latter is due to parameter settings? what about MVS methods that use learning only for components, e.g., depth map computation or predicting uncertainty for the depth, these are the current state of the art on tanks and temples and eth 3d.}.
However, all of these methods require a long optimization time and are limited to small scenes focusing on reconstructing single objects. %
\torsten{maybe the latter is due to parameter settings? what about MVS methods that use learning only for components, e.g., depth map computation or predicting uncertainty for the depth, these are the current state of the art on tanks and temples and eth 3d.}. 

Most recently, another line of research~\cite{Sun2021ARXIV,Yu2021cARXIV,Muller2022ARXIV} significantly reduces the training time of NeRF by replacing the large (MLP) with either dense voxel grids or a lightweight MLP conditioned on features distributed on a spatial 3D grid, which is cheap to query using trilinear interpolation. While these methods achieve comparable or even better novel view synthesis results compared to NeRF, and can represent sophisticated object shapes when dense 3D supervision are avaliable (\ie Instant-ngp~\cite{Muller2022ARXIV} and NGLOD~\cite{takikawa2021nglod}), it remains unclear how effective they can be as a general-purpose neural implicit surface representation trained only on multi-view RGB images as input. 

In this work, we propose \textit{InstantSDF}, a neural implicit field conditioned on a multi-resolution feature grid \michael{change name? If so, not only inspired by Instant NGP}.
InstantSDF enables detailed large-scale 3D reconstruction from only multi-view posed images while also being more efficient to train compared to previous approaches. \torsten{I wouldn't call it large-scale since we are still looking at rather small scenes. Medium-scale might be more accurate. I would reserve large-scale for larger outdoor scenes. Also, wasn't there some work by NVidia on implicit neural representations for larger scenes? Also, BlockNerf handles larger scenes as well.} 
Our key observation is that a single, large MLP is insufficient to represent high-detail geometry while being computational expensive to evaluate and optimize. \torsten{Isn't this also what other work does? E.g., BlockNerf uses multiple NeRFs.}
In contrast, a high-resolution signed distance grid is cheap to evaluate with trilinear interpolation.
However, in contrast to an MLP-based representation, gradient updates only affect the local grid cell and have no influence on neighbouring areas. As a result, the optimization is more local leading to noisy geometry predictions in less-observed areas.
Using a small MLP together with a feature grid is a compromise between the two extremes.
While it is comparably efficient to optimize and evaluate due to the feature grid, it utilizes a shared MLP for all feature grid cells, thereby inheriting the favorable inductive biases of MLP-based representations.
However, this combination alone still leads to noisy geometry predictions with block-like artifacts as only a single, high-frequency grid is used.
Instead, we propose to combine grid features from multiple resolutions leading to an automatic balance of low and high frequencies and provide a detailed analysis of the unique properties of multi-resolution grids. \torsten{Didn't the Instant-NGP paper already use a multi-res grid?}
In contrast to existing works that suggest using a small MLP for SDF prediction, we found such a design produce noise meshes in our taks of multi-view reconstruction. Simply increasing the hidden dimension of the MLP brings more smoothness. However, applying it to larger room-level scenes such as the Replica dataset fails because only a subset of voxel grid is updated at each iteration and by setting a relatively larger learning rate for the feature grid significantly improve the results.

\begin{itemize}
    \item We present Instant SDF, a neural implicit surface reconstruction method utilizing multi-resolution feature grids. Our method enables detailed 3D reconstruction of large-scale scenes and is more efficient to optimize compared to state-of-the art implicit surface reconstruction methods. We provide a detailed analysis and deepened understanding of the effect of the multi-resolution feature grids.
    
    \item We validated the effectiveness, efficiency and scalability of our Instant-SDF on  the DTU dataset\cite{Aanes2016IJCV} and the Replica dataset\cite{Knapitsch2017SIGGRAPH}). We observe that our method yields higher geometric quality while converging faster than competing methods.
\end{itemize}



\section{Introduction2 - Monocular geometric priors}
3D reconstruction from multi-view images is a fundamental problem in computer vision with  well-established applications such as graphics, animation, virtual reality, and more. Recently, neural radiance fields (NeRFs)~\cite{Mildenhall2020ECCV} have shown impressive results on the task of novel view synthesis by using multi-layer perceptrons (MLPs) in combination with volume rendering techniques. Building on NeRF, several works~\cite{Oechsle2021ICCV,Wang2021NEURIPS,Yariv2021NEURIPS} investigate how proposed techniques can be used for the task of 3D reconstruction and they introduce new ways \torsten{"new ways" sounds a bit handwavy, can we be more precise?} of modelling volume density as a function of the underlying 3D surface, which in turn improves optimized scene geometry. 
For example, in UNISURF~\cite{Oechsle2021ICCV} NeRF's density field is replaced by an occupancy field, while in NeuS~\cite{Wang2021ARXIVb} and VolSDF~\cite{Yariv2021NEURIPS} the density field is modeled with a signed distance field instead.
These methods show improved surface reconstruction quality compared to NeRF and the extracted meshes are smoother and more complete compared to traditional methods like COLMAP~\cite{Schoenberger2016CVPR} \torsten{maybe the latter is due to parameter settings? what about MVS methods that use learning only for components, e.g., depth map computation or predicting uncertainty for the depth, these are the current state of the art on tanks and temples and eth 3d.}. 
However, all of these methods require a long optimization time and are limited to small scenes focusing on reconstructing single objects. %
\torsten{I think this paragraph jumps into details too quickly. I think it would be good to stay on a high level here and go into details in the next paragraph.}

The core of these method is the differentiable volume rendering where a pixel value is rendered and optimized with multi-view RGB images. However, there is inherent ambiguity for the such a reconstruction loss especially for reflections, specularities, and  textureless or rarely observed regions. To address this problem, we need a higher level understanding of the scene. For example, the wall in a room should be flat and straight. Recently, generalizable single view depth prediction and normal prediction make a huge progress and to our surprise\torsten{"to our surprise" sounds a bit colloquial. I think there are reasons why these have not been exploited: up to recently, the depth was often severely distorted, making the depth maps hard to use, at least in general scenes. We should try to explain why these haven't been used before}, it's not fully exploited in the context of neural surface reconstruction \torsten{"it's not fully exploited" sounds like it has been used before. Is this the case? And if so, how and how does our work differ?}. Therefore, in this paper, we investigate how these neural implicit method can benefits from monocular geometric priors. Specifically, we extract monocular geometric priors (\ie depth and surface normal) for each image and used it as an additional supervision for our optimization. We found a natural \torsten{what does natural mean?} incorporation of monocular prior improve the reconstruction quality and efficiency significantly. \torsten{I guess we need the disclaimer that this holds for more complex scenes.}

Most recently, another line of research~\cite{Sun2021ARXIV,Yu2021cARXIV,Muller2022ARXIV} significantly reduces the training time of NeRF by replacing the large MLP with either dense voxel grids or a lightweight MLP conditioned on features distributed on a spatial 3D grid, which is cheap to query using trilinear interpolation. While these methods achieve comparable or even better novel view synthesis results compared to NeRF, and can represent sophisticated object shapes when dense 3D supervision are avaliable (\ie Instant-ngp~\cite{Muller2022ARXIV} and NGLOD~\cite{takikawa2021nglod}), it remains unclear how effective they can be as a general-purpose neural implicit surface representation trained only on multi-view RGB images as input. \TS{This seems a bit vague, can we at least explain why they are unlikely to handle more complex / larger scenes?} \torsten{in the new story line, this seems unnecessary. Maybe move to the related work section?}

Inspired by these works, we investigated different kinds of scene representation and conducted extensive experiments. Our key observation is that a single, large MLP is insufficient to represent high-detailed geometry while being computational expensive to evaluate and optimize. In contrast, a high-resolution signed distance grid is cheap to evaluate with trilinear interpolation. However, in contrast to an MLP-based representation, gradient updates only affect the local grid cell and have no influence on neighbouring areas. As a result, the optimization is more local leading to noisy geometry predictions in less-observed areas. Using a small MLP together with a feature grid is a compromise between the two extremes. While it is comparably efficient to optimize and evaluate due to the feature grid, it utilizes a shared MLP for all feature grid cells, thereby inheriting the favorable inductive biases of MLP-based representations.
However, this combination alone still leads to noisy geometry predictions with block-like artifacts as only a single, high-frequency grid is used. Instead, combining grid features from multiple resolutions leading to an automatic balance of low and high frequencies. 
\torsten{This part seems a bit disconnected from the priors part. Also, it is missing some point explaining how we overcome the limitations of prior work.}

In summary, we make the following contributions:

\begin{itemize}
    \item We introduce a general monocular geometric prior to improve the reconstruction quality and efficiency of neural implicit models. It enables detailed 3D reconstruction of large-scale scenes and is more efficient to optimize compared to state-of-the art implicit surface reconstruction methods. 
    \item We investigate and analyze several design choice of neural implicit surface representation. We provide systematic comparison and detailed analysis of different representations. We found the pure mlp based representation is more robust to imperfect geometric prior while the multi-resolution gird can recover more detailed geometry but also has more noise.
    \item We validated the effectiveness, efficiency and scalability of our method on the multiple challenging datasets, ranging from laboratory captured dataset(\ie the DTU dataset\cite{Aanes2016IJCV}) to large scale scenes (\ie the Tanks and Temples dataset\cite{Knapitsch2017SIGGRAPH}). We observe that our method yields higher geometric quality while converging faster than competing methods.
\end{itemize}
